Intersection graph of maximal stars

A biclique of a graph $G$ is an induced complete bipartite subgraph of $G$ such that neither part is empty. A star is a biclique of $G$ such that one part has exactly one vertex. The star graph of $G$ is the intersection graph of the maximal stars of $G$. A graph $H$ is star-critical if its star graph is different from the star graph of any of its proper induced subgraphs. We begin by presenting a bound on the size of star-critical pre-images by a quadratic function on the number of vertices of the star graph, then proceed to describe a Krausz-type characterization for this graph class; we combine these results to show membership of the recognition problem in \textsf{NP}. We also present some properties of star graphs. In particular, we show that they are biconnected, that every edge belongs to at least one triangle, characterize the structures the pre-image must have in order to generate degree two vertices, and bound the diameter of the star graph with respect to the diameter of its pre-image. Finally, we prove a monotonicity theorem, which we apply to list every star graph on at most eight vertices.

==> secoes/squareold.tex <==
\section{Star graph of triangle-free graphs}


\begin{figure}[!htb]
    \centering
    
        \begin{tikzpicture}[rotate=45,scale=\gscale]
            
                \GraphInit[unit=3,vstyle=Normal]
                %\draw[help lines] (-5,-5) grid (5,5);
                \SetVertexNormal[Shape=circle, FillColor=black, MinSize=2pt]
                \tikzset{VertexStyle/.append style = {inner sep = \inners, outer sep = \outers}}
                \begin{scope}[shift={(-2.41cm, 0cm)}]
                    \SetVertexNoLabel
                    \grEmptyCycle[RA=1.41,prefix=a]{4}
                    \Edges(a0,a1,a2,a3,a0)
                    \Vertex[x=0,y=2.41]{1a}
                    %\Vertex[y=0,x=-2.41]{2a}
                    \Vertex[x=0,y=-2.41]{3a}
                    \Edge(1a)(a1)
                    %\Edge(2a)(a2)
                    \Edge(3a)(a3)
                \end{scope}
                \begin{scope}[shift={(2.41cm, 0cm)}]
                    \SetVertexNoLabel
                    \grEmptyCycle[RA=1.41,prefix=b]{4}
                    \Edges(b0,b1,b2,b3,b0)
                    \Vertex[x=0,y=2.41]{1b}
                    %\Vertex[y=0,x=2.41]{0b}
                    \Vertex[x=0,y=-2.41]{3b}
                    \Edge(1b)(b1)
                    %\Edge(0b)(b0)
                    \Edge(3b)(b3)
                \end{scope}
                \Edge(a0)(b2)
        \end{tikzpicture}
        \hfill
        \begin{tikzpicture}[rotate=45,scale=\gscale]
            
                \GraphInit[unit=3,vstyle=Normal]
                %\draw[help lines] (-5,-5) grid (5,5);
                \SetVertexNormal[Shape=circle, FillColor=black, MinSize=2pt]
                \tikzset{VertexStyle/.append style = {inner sep = \inners, outer sep = \outers}}
                \begin{scope}[shift={(-2.41cm, 0cm)}]
                    \SetVertexNoLabel
                    \grEmptyCycle[RA=1.41,prefix=a]{4}
                    \Edges(a0,a1,a2,a3,a0)
                    \Vertex[x=0,y=2.41]{1a}
                    %\Vertex[y=0,x=-2.41]{2a}
                    \Vertex[x=0,y=-2.41]{3a}
                    \Edge(1a)(a1)
                    %\Edge(2a)(a2)
                    \Edge(3a)(a3)
                    
                    \Edge(a0)(a2)
                    \Edge(a1)(a3)
                    
                    \Edge(1a)(a2)
                    \Edge(3a)(a2)
                    \Edge(1a)(a0)
                    \Edge(3a)(a0)
                    %\Edge(2a)(a1)
                    %\Edge(2a)(a3)
                \end{scope}
                \begin{scope}[shift={(2.41cm, 0cm)}]
                    \SetVertexNoLabel
                    \grEmptyCycle[RA=1.41,prefix=b]{4}
                    \Edges(b0,b1,b2,b3,b0)
                    \Vertex[x=0,y=2.41]{1b}
                    %\Vertex[y=0,x=2.41]{0b}
                    \Vertex[x=0,y=-2.41]{3b}
                    \Edge(1b)(b1)
                    %\Edge(0b)(b0)
                    \Edge(3b)(b3)
                    
                    \Edge(b0)(b2)
                    \Edge(b1)(b3)
                    
                    \Edge(1b)(b2)
                    \Edge(3b)(b2)
                    \Edge(1b)(b0)
                    \Edge(3b)(b0)
                    %\Edge(0b)(b1)
                    %\Edge(0b)(b3)
                \end{scope}
                \Edge(a0)(b2)
                \Edge(a0)(b1)
                \Edge(a0)(b3)
                \Edge(b2)(a1)
                \Edge(b2)(a3)
        \end{tikzpicture}
        \hfill
        \begin{tikzpicture}[shift={(1.41cm,0cm)},rotate=45,scale=\gscale]
            
                \GraphInit[unit=3,vstyle=Normal]
                %\draw[help lines] (-5,-5) grid (5,5);
                \SetVertexNormal[Shape=circle, FillColor=black, MinSize=2pt]
                \tikzset{VertexStyle/.append style = {inner sep = \inners, outer sep = \outers}}
                \begin{scope}[shift={(-2.41cm, 0cm)}]
                    \SetVertexNoLabel
                    \grEmptyCycle[RA=1.41,prefix=a]{4}
                    \Edges(a0,a1,a2,a3,a0)
                    \Edge(a0)(a2)
                    \Edge(a1)(a3)
                \end{scope}
                \begin{scope}[shift={(2.41cm, 0cm)}]
                    \SetVertexNoLabel
                    \grEmptyCycle[RA=1.41,prefix=b]{4}
                    \Edges(b0,b1,b2,b3,b0)
                    \Edge(b0)(b2)
                    \Edge(b1)(b3)
                \end{scope}
                \Edge(a0)(b2)
                \Edge(a0)(b1)
                \Edge(a0)(b3)
                \Edge(b2)(a1)
                \Edge(b2)(a3)
        \end{tikzpicture}
        \hfill
    
    
    
    \caption{A triangle-free graph (left), its square (center) and its star graph (right).}
    \label{fig:tri_star}
\end{figure}



In this section we will interpret star graphs in terms of powers of graphs and give an $\NPcness$ reduction for the recognition of a subclass of star graphs.

\begin{observation}
    Every vertex of degree at least two in a triangle free graph is the center of exactly one maximal star.
\end{observation}

\begin{theorem}
    \label{thm:tri_free_star}
    If $H$ is a $K_3$-free graph with at least 3 vertices, $D$ are its vertices of degree at least 2 and $G = \K{S}(H)$, it holds that $G \simeq H[D]^2$.
\end{theorem}

\begin{tproof}
    There are only 4 graphs $H$ with at most 4 vertices that are triangle free, namely $P_3, K_{1,3}, P_4, C_4$, which have star graphs equal to $K_1, K_1, K_2, K_4$, respectively, and clearly satisfy the property.
    We restrict our analysis to graphs of order at least 5, and define $L = V(H) \setminus D$.
    This constraint implies that every star has at least 3 vertices.
    
    The previous observation trivially guarantees that $|V(G)| = |D| = |V(H)| - |L| = |V(H^2)| - |L|$, since the only vertices of $H$ that do not have a maximal star centered around them are precisely the ones with degree 1 and every other is the center of exactly 1 maximal star.
    Consequently, we can safely build a bijection $f : D \mapsto V(G)$, where $f(v_i) = a$ if and only if the center of $s_a$, the maximal star of $H$ correspondent to $a$, is $v_i$.
    
    First, to show that $E(G) \subseteq E(H[D]^2)$, take an edge $ab \in E(G)$ and the corresponding stars $s_a, s_b \in \str(H)$.
    By the definition of $G$, $s_a \cap s_b \neq \emptyset$. If $|s_a \cap s_b| = 2$, clearly $f(a)^{-1}f(b)^{-1} \in E(H)$ and it follows that $f^{-1}(a)f^{-1}(b) \in E(H[D]^2)$.
    Otherwise, since there is only one maximal star centered on each vertex of $H$, we have that $v_i = f^{-1}(a) \neq f^{-1}(b) = v_k$ and there is at least one $v_j \in s_a \cap s_b$.
    Therefore, $v_j \in N_H(v_i) \cap N_H(v_k)$ and $v_iv_k \notin E(H)$ since $H$ is $K_3$-free, from where we conclude that $v_iv_jv_k$ is an induced $P_3$ of $H$ and, consequently, $\dist(v_i, v_k) = 2$, which implies that $v_iv_k \in E(H[D]^2)$, that is, $f^{-1}(a)f^{-1}(b) \in E(H[D]^2)$.
    
    For $E(H[D]^2) \subseteq E(G)$, take an edge $v_iv_k \in E(H[D]^2)$ but $v_iv_k \notin E(H)$.
    Because $v_i,v_k \in D$, there is $s_a \in \str(H)$ corresponding to $a = f(v_i)$ and $s_b \in \str(H)$ corresponding to $b = f(v_k)$ with $v_j \in s_a \cap s_b$ and, consequently, $ab \in E(G)$, that is, $f(v_i)f(v_k) \in E(G)$. Otherwise, if $v_iv_k \in E(H)$, $f(v_i)f(v_k) \in E(G)$ trivially holds since $\{v_i,v_k\} = s_a \cap s_b$.
\end{tproof}

\begin{corollary}
    If $H$ is $K_3$-free with  $\delta(H) \geq 2$, then $\K{S}(H) \simeq H^2$.
\end{corollary}

The above characterization gives a nice way to think about star graphs as the square of triangle free graphs with minimum degree 2.
If the pre-image is also $C_4$-free, we have an analogous characterization for the biclique graph.

\begin{corollary}
    If $H$ is $\{K_3, C_4\}$-free, $\delta(H) \geq 2$ and $G = \K{B}(H)$, $G \simeq H^2$.
\end{corollary}

Nguyen~\citep{girth_powers} extensively studied powers of graphs of constrained girth, giving a polynomial time algorithm for 

\problem{square of graph with girth $\geq 6$}{A graph $G$}{Is there an $H$ with $\girth(H) \geq 6$ such that $G \simeq H^2$?}
\newline
and an $\NPcness$ proof for

\problem{square of graph with girth $\leq 4$}{A graph $G$}{Is there an $H$ with $\girth(H) \leq 4$ such that $G \simeq H^2$?}

The given proof shows that \textsc{square of graph with girth $= 4$} is $\NPc$, and, using the fact that \textsc{square of graph with girth $= 3$} is $\NPc$, a result given by~\citep{hard_roots}, it is concluded that \textsc{square of graph with girth $\leq 4$} is $\NPc$.

As such, using Theorem~\ref{thm:tri_free_star} and the polynomial time algorithm for \textsc{square of graph with girth $\geq 6$}, we obtain the following result.

\begin{theorem}
    Given a star graph $G$, there is a polynomial time algorithm that checks if there exists a triangle-free graph $H$ with girth at least 6 such that $G \simeq \K{S}(H)$.
\end{theorem}

Since graphs of girth exactly four are triangle-free, these hardness results point toward the $\NPcness$ of \textsc{star graph} of triangle-free graphs.
We state a particular case of \textsc{star graph} in terms of girth of the pre-image and establish its $\NPcness$ in the following theorem.

\problem{star graph of graph with girth $= 4$}{A graph $G$}{Is there an $H$ with $\girth(H) = 4$ such that $G \simeq \K{S}(H)$?}

\begin{theorem}
    \textsc{star graph of graph with girth $= 4$} is $\NPc$.
\end{theorem}

\begin{tproof}
    Due to Theorem~\ref{thm:tri_free_star}, membership in $\NP$ is easily verified.
    For our reduction, we will use \textsc{square of graph with girth $= 4$} and suppose that all graphs used in this proof are connected.
    We denote by $G$ and $H$ the input and output of \textsc{square of graph with girth $= 4$}, respectively, and by $G'$ and $H'$ the input and output to \textsc{star graph of graph with girth $= 4$}.
    Our instance $G$ is exactly as $G'$, that is, $G = G'$.
    
    First, take a solution $H$ to \textsc{square of graph with girth $= 4$} and build $H'$ with $V(H') = V(H) \cup \{u' \mid u \in V(H)\}$ and $E(H') = E(H) \cup \{uu' \mid u \in V(H)\}$.
    That is, $H$ is an induced subgraph of $H'$ obtained by removing every vertex $u'$ of degree one.
    We denote such set by $U(H')$ and the remaining vertices by $D(H') = V(H') \setminus U(H') = V(H)$.
    Note that $H'$ also has girth 4 because $H$ has girth 4 and no $u' \in U(H')$ is contained in a cycle of $H'$ nor induces a triangle.
    Using Theorem~\ref{thm:tri_free_star}, we conclude that $G' = G = H^2 = \left(H' \setminus U(H')\right)^2 = H'[D(H')]^2 = \K{S}(H')$.
    
    For the converse, take a solution $H'$ to \textsc{star graph of graph with girth $= 4$}, denote by $D(H')$ its vertices of degree at least 2 and take $H = H'[D(H')]$.
    Clearly, $H$ has girth 4 and remains connected.
    Using Theorem~\ref{thm:tri_free_star} we conclude that $G = G' = \K{S}(H') = H'[D(H')]^2 = H^2$.
\end{tproof}


Nguyen~\citep{girth_powers} conjectures that \textsc{square of graph with girth $= 5$} is polynomially solvable, which partially reduces the motivation to study the star graph of $\{K_3, C_4\}$-free graphs, as it may not aid in a proof for the complexity of biclique graph recognition.
